Towards Zero-Shot Functional Compositionality of Language Models

Large Pre-trained Language Models (PLM) have become the most desirable starting point in the field of NLP, as they have become remarkably good at solving many individual tasks. Despite such success, in this paper, we argue that current paradigms of working with PLMs are neglecting a critical aspect of modeling human intelligence: functional compositionality. Functional compositionality - the ability to compose learned tasks - has been a long-standing challenge in the field of AI (and many other fields) as it is considered one of the hallmarks of human intelligence. An illustrative example of such is cross-lingual summarization, where a bilingual person (English-French) could directly summarize an English document into French sentences without having to translate the English document or summary into French explicitly. We discuss why this matter is an important open problem that requires further attention from the field. Then, we show that current PLMs (e.g., GPT-2 and T5) don't have functional compositionality yet and it is far from human-level generalizability. Finally, we suggest several research directions that could push the field towards zero-shot functional compositionality of language models.

==> contents/ResponsibleNLP.tex <==
\section{ResponsibleNLP}
In this paper, we explore whether PLMs can compose the functions that they already learned. 
\sout{Our empirical results suggest that 1) PLMS cannot compose as it is, but can learn how to compose, 2) it can be achieved even with fewer parameters, and 3) it cannot be transferred between different datasets (from style transfer to cross-lingual summarization).}
\mh{Our empirical results suggest that 1) PLMS cannot compose as it is, 2) but it can be partially done by learning-to-compose (L2C), and 3) the learned compositional skill is limited so that it cannot be transferred between different benchmarks (from style transfer to cross-lingual summarization). }
From the results, we suggest several future research directions to explore further generalization of its ability to other tasks (\eg, bias-free generation and cross-lingual classification) and training stages (\eg, pre-training and few-shot fine-tuning).

==> contents/backup.tex <==
% \section{Problem Formulation}
% Task definition


% Complex RL problems can often be divided into easier subproblems. 
% Recent yearss have taught us that, given unlimited experience, artificial agents can tackle such complex problems without any sense of their compositional structures. 
% However, discovering the underlying subproblems and learning to solve those would enable learning with substantially less experience, especially when faced with numerous tasks that share common structure.
% While our work shares this premise with iherarchical RL efforts, those works do not consider the formulation we present here, where functional composition occurs at multiple hierarchical levels of abstraction. 

% An RL problem is a composition of subproblems F1, F2, ... if its optimal policy phi* can be constructed by combining solutions to those subproblems: phi*(s) = m1 * m2 * ... , where each mi is the solution to the corresponding Fi. 

% In lifelong compositional RL, the agent will be faced with a sequence of MDPs over its lifetime. 
% We assume that all MDPs are compositions of different subsets from k shared subproblems. 
% The goal of the lifelong learner is to find the set of solutions to these subproblems as a set of modules, such that learning to solve a new problem reduces to finding how to combine these modules optimally. 
% Each module can be viewed as a processing stage in a hierarchical processing pipeline, or equivalently as functions in a program, and the goal of the agent is to find the correct module to execute at each stage and the instantiation of that module (i.e., its parameters). 

% Formally, we assume that the descriptor is given as an external input, and that there exists some function s that can map this input and an optimal set of modules into an optimal policy for the current task s. This would enable the agent to achieve compositional generalization: the ability to solve a new task entirely by reusing components learned from previous tasks. 

% \subsection{Functional Compositionality for Style Transfer}
% \cite{lyu2021styleptb} introduces compositions of multiple transfers which allow modeling of fine-grained stylistic changes as building blocks for more complex, high-level transfers. 
% and find that existing methods struggle to model fine-grained changes and have an even more difficult time composing multiple styles. 
% controllable text style transfer, compositional models, and learning disentangled representations. 
% Solving these challenges would present important steps towards controllable text generation.
% can in fact be seen as composed from a dictionary of fine-grained style constructs. This alternative way of studying styles brings additional flexibility that enables fine-grained control with the possibility to compose a broader space of styles spanning tense, sentence structure, phrase emphasis, and information contained in the sentence. 
% study formulations of styles across 4 representational categories: lexical, syntax, semantics, and thematics, that span the fundamental atomic transfers that text can undergo. 
% To allow for compositionality, we also generated compositional data that includes parallel pairs of sentences linked by multiple sequential transfers. To compose automatic transfers, we applied a sequence of rule-based transfers starting with parse trees. To compose transfers that involve human annotations, we apply a sequence of ``reverse'' changes on the original sentences with parse trees (since human rewritten sentences no longer have parse trees), before chaining the sequence of automatic reverse transfers with the final human-annotated transfer. 

% \hist{...}
% Firstly, suppose there are $N$ component tasks $\mathcal{T}_1, \ldots, \mathcal{T}_N$. 
% Then, we can assume there are $M$ tasks, where each of them is a functional composition of two component tasks, \ie, $\mathcal{T}_{i \rightarrow j}(x)$ = $\mathcal{T}_{j} (\mathcal{T}_{i}(x))$. 
% Our research question is thus, after training the $N+M$ tasks, can the model generalize to unseen $M+1$-th composition task?


% For training, on frozen pre-trained parameters $\theta_0$, we update only the task-specific parameters $\theta_{\mathcal{T}}$ on the following log-likelihood objective:
% \begin{align}
%     \max_{\theta_0, \theta_{\mathcal{T}}} \log p_{\theta_0, \theta_{\mathcal{T}}} (y | x) = \sum_{i \in Y_{idx}} \log p_{\theta_0, \theta_{\mathcal{T}}} (z_i | h_{<i}).
% \end{align}

% For training, we perform gradient updates on the log-likelihood objective, where the language model parameters $\phi$ are fixed and the prefix parameters $\theta$ are the only trainable parameters: 
% \begin{align}
%     \max_{\theta} \log p_{\theta} (y | x) = \sum_{i \in Y_{idx}} \log p_{\theta} (z_i | h_{<i}).
% \end{align}


% \input{figures/placeholder_big}



% Here, $h_i$ (for all $i$) is a function of the trainable $P_{\theta}$. When $i \in P_{\text{idx}}$, this is clear because $h_i$ copies directly from $P_{\theta}$. 
% When $i \notin P_{\text{idx}}$, $h_i$ still depends on $P_{\theta}$, because the prefix activations are always in the left context and will therefore affect any activations to its right.

% \hist{copied from prefix}
% Empirically, directly updating the $P_{\theta}$ parameters leads to unstable optimization and a slight drop in performance. 
% So we reparametrize the matrix $P_{\theta}[i, :] = MLP_{\theta}(P'_{\theta}[i, :])$ by a smaller matrix ($P'_{\theta}$) composed with a large feedforward neural network ($MLP_{\theta}$). 
% Note that $P_{\theta}$ and $P'_{\theta}$ has the same rows dimension (\ie, the prefix length), but different columns dimension. 
% Once training is complete, these reparametrization parameters can be dropped, and only the prefix ($P_{\theta}$) needs to be saved. 





% ====== ======= ======= ======== Move below to appendix maybe? ======= ======= ======= =======


% \subsection{Preliminaries: Prefix Tuning}
% Prefix-tuning \cite{li2021prefix} prepends a prefix for an autoregressive LM to obtain $z = [\textsc{Prefix}; x; y]$, or prepends prefixes for both encoder and encoder to obtain $z = [\textsc{Prefix}; x; \textsc{Prefix'}; y]$, as shown in Figure~\ref{fig:architecture}.
% Here, $P_{\text{idx}}$ denotes the sequence of prefix indices, and we use $|P_{\text{idx}}|$ to denote the length of the prefix.
% Prefix-tuning initializes a trainable matrix $P_{\theta}$ (parametrized by $\theta$) of dimension $|P_{\text{idx}}| \times \text{dim}(h_i)$ to store the prefix parameters.
% \begin{align}
%     h_i = \begin{cases}
%             MLP_{\theta}(P_{\theta}[i,:]), & \text{if } i \in P_{\text{idx}}, \\
%             \text{LM}_{\phi}(z_i, h_{<i}), & \text{otherwise},
%         \end{cases}
% \end{align}
% where $MLP_{\theta}$ is a reparametrization technique, employed to make optimization of $P_{\theta}$ more stable as in~\cite{li2021prefix}. 


% This section discusses the overall architecture of our proposed method, illustrated in Figure~\ref{fig:architecture}, which is based on prefix tuning~\cite{li2021prefix} with an introduction of (1) shared encoder and (2) composer module. 
% On the architecture, we will describe how our learning algorithm can perform the functional composition of the component tasks. 
% \subsection{Shared Encoder \& Composer}

% Prefix tuning~\cite{li2021prefix} avoids catastrophic forgetting by introducing task-specific parameters, but it makes functional composition difficult because the representation spaces are not aligned between multiple tasks. 
% Therefore, it is required to align the representation between spaces while keeping the task-specific parameters. 
% Though similar discussions are observed in~\cite{pfeiffer2021adapterfusion}, updating the pre-trained weights $\phi$, our distinction is keep the pre-trained weights $\phi$ and still performs parameter-efficient fine-tuning. 

% For the sake of this discussion and with out loss of generality, we will consider a decomposition of the prefix modules into two learnable parameters - a prefix vector and an encoder network, as shown in Figure~\ref{fig:architecture}. 
% The former learns how to perform a task itself, and latter focuses more on learning how to transform the task-specific knowledge into layer-wise one. 
% A distinction from original implementation is that we share the encoder network between the multiple tasks, for the purpose of aligning the representation spaces. 


% \subsection{Learning Algorithm}

% For this purpose, we propose a two-stage training algorithm based on prefix tuning~\cite{li2021prefix}, where the first stage yields $N$ different prefix vectors trained on the $N$ component tasks, and the second stage only learns how to compose the prefix vectors on the $M$ composition tasks. 

% In the \textbf{first stage}, we train the prefix vectors of $N$ component tasks. Specifically, to avoid catastrophic forgetting in the encoder module, we feed

% \hist{overview: 1. prefix-tuning on component tasks with shared encoder. 2. training attentions (of component tasks) on composition tasks. 3. evaluating zero-shot composition of seen component tasks.}


% \hist{1) we first train prefix vectors of $N$ component tasks. specifically, we share the encoder network among the component tasks, hoping the encoder network to learn how to distribute the prefix vectors into the transformer layers. 2) after fixing prefix vectors and the encoder network, we train the composer network with the $M$ composition tasks. 3) at test time, for $M+1$-th composition task, we feed the prefix vectors of its component tasks.}

% \subsection{Composer}


% Recent auto-regressive PLMs like T5 have shown great progress in prompt-based methods worked good in few-shot and zero-shot! Amazing!
% However, as we have seen earlier, current PLMs fail to generalize compositionally
% Hence, we attempt to teach compositionality to our PLMs through compositional prompts
% We try two different ways to do so:
% 1. Natural Language Instructions (e.g. Remove all prepositional phrases and change to future tense.)
% 2. Simplified instructions (e.g. ``TFU + PPR'')

% \mh{As a prompt is consist of natural language instruction, The natural way to compose two atomic task prompts is rewriting a composition task prompt based on the atomic task prompts. However, in our preliminary experiments, significant performance drop occurs in some composition tasks when we rewrite prompts by human. The possible cause is that model is faced with unseen patterns in some special tasks. So, we simplify instruction for both atomic task and composition task. (e.g. ``TFU + PPR'' as a composition of ``To Future Tense without all prepositions'') }

% \mh{Specifically, we map a single token as a atomic task prompt. For example, ``To Future Tense'' and ``Remove All Prepositions'' tasks are mapped to ``TFU'' and ``PPR'', respectively. After that, we define a composition task prompt as a sequential combination with `+' operator. (e.g. ``TFU + PPR'') we concatenate the simplified prompt with each task input, and train the model with the prompted inputs. To avoid catastrophic forgetting of atomic tasks, we train the model with the composition tasks along with its atomic tasks in multi-task manner, which motivates non-destructive compositions with task-specific parameters as we will discuss later (Section~\ref{}).}
% examples of prompt compositions: maybe figures?
% \input{figures/placeholder_small}


%(\ie `To Future (TFU)', `To Present (TPR)', `To Past (TPA)', `Active to Passive (ATP)', `Passive to Active(PTA)', `PP Front to Back (PFB)', `PP Back to Front (PBF)', `ADJ/ADV Removal (ARR)', `PP Removal (PPR)').

%To confirm convergence, we use 10\% of the train set for validation purposes. The learning parameters were chosen by the best performance on the validation set.

% \noindent\textbf{Prompt Fine-Tuning} As a naive fine-tuning cannot perform unseen tasks, we consider the prompt fine-tuning \cite{han2021ptr} as baseline, giving natural language instructions to T5, like ``translate this document into French'' ($x \rightarrow y$) or ``summarize this document'' ($y \rightarrow z$).
% For the composition task $x \rightarrow z$, we construct manual instructions of naturally summarizing the component tasks at once, such as such as ``summarize this document into French sentence''\footnote{We also tried other variants of automatic prompt-level compositions, like ``first [translate this document into French], then [summarize the document]''. but the manual instruction performs the best.}. 
% The prefix texts used in this work are listed in Appendix~\ref{}. 

% \hist{copied from \cite{zhang2021differentiable}.}
% Formally, let $X_{\text{in}} = \{x_{1}, x_{2},..., x_{L}\}$ be a sentence, where $x_{i}$ is the $i$-th token in the input sentence and $L$ is the number of tokens. Specifically, $X_{\text{in}}$ is converted to a fixed token sequence $\tilde{X}_{\text{in}}$ and then mapped to a sequence of hidden vectors $\{\mathbf{h}_{k} \in \mathbb{R}^{d}\}$. 
% Given the input sequence, $\tilde{X}_{\text{in}} = \texttt{[CLS]} X_{\text{in}} \texttt{[SEP]}$, the
% conventional fine-tuning approaches leverage a generic head layer over [CLS] embeddings (e.g., an
% MLP layer) to predict an output class. 
% For the prompt-based method, a task-specific pattern string (template $\mathcal{T}$) is designed to coax the model into producing a textual output corresponding to a given
% class (label token $\mathcal{M}(Y)$)- we refer to these two things together as a prompt. Specifically, $X_{\text{prompt}}$
% containing one [MASK] token is directly tasked with the MLM input as:
% \begin{align}
%     X_{\text{prompt}} = \texttt{[CLS]}X_{\text{in}}\texttt{[SEP]}T\texttt{[SEP]}
% \end{align}
% When the prompt is fed into the MLM, the model can obtain the probability distribution $p(\texttt{[MASK]}|(X_{\text{prompt}})$ of the candidate class, $y \in Y$ as:
% \begin{align}
%     p(y|X_{\text{prompt}}) = \sum_{w \in \mathcal{V}_{y}} p(\texttt{[MASK]} = w|X_{\text{prompt}})
% \end{align}
% where $w$ represents the $w$-th label token of class $y$.

% \noindent\textbf{Pipeline}: 
% 1. annotation efficient
% 2. computationally expensive
% 3. error propagation from former task

==> figures/placeholder_big.tex <==
\begin{figure*}[!t]
  \centering
  \includegraphics[draft,clip,width=0.95\textwidth]{figures/architecture.png}
  \caption{Placeholder big}
\end{figure*}

==> figures/placeholder_small.tex <==
\begin{figure}[!t]
  \centering
  \includegraphics[draft,clip,width=0.45\textwidth]{figures/architecture.png}
  \caption{Placeholder small}
\end{figure}

==> tables/tab_full_depricated.tex <==
\begin{table*}[t!]
\begin{center}
\begin{adjustbox}{angle=90}
\begin{tabular}{llccccccccccc}
  \hline
  \noalign{\hrule height0.8pt} %%%%=
  \multicolumn{1}{l}{\multirow{2}{*}{}} & 
  \multicolumn{1}{l}{\multirow{2}{*}{Model}} &
  \multicolumn{11}{c}{Target Composition} \TBstrut\\
  \cline{3-13}
  & & TFU+ATP & TFU+PTA & TFU+PPR & TPR+ATP & TPR+PTA & TPR+PPR & TPA+ATP & TPA+PTA & TPA+PPR & ATP+PPR & PTA+PPR \TBstrut\\
  \hline\noalign{\hrule height0.8pt} 
  \multirow{2}{*}{\textbf{Full-shot}} 
  & \textsc{Fine-Tune} & 0.7984 & 0.8605 & 0.8818 & 0.7949 & 0.8511 & 0.8529 & 0.6286 & 0.8800 & 0.8571 & 0.7664 & 0.8000 \TBstrut \\
  & \textsc{Prefix} & 0.7054 & 0.7597 & 0.8276 & 0.6410 & 0.7660 & 0.8162 & 0.5714 & 0.8267 & 0.8312 & 0.6642 & 0.7375 \TBstrut \\
  \hline\noalign{\hrule height0.8pt} 
  
  \multirow{4}{*}{\textbf{Zero-shot}} 
  & \textsc{Fine-Tune} & 0.8062 & 0.8140 & 0.8867 & 0.7821 & 0.8085 & 0.8750 & 0.4857 & 0.8800 & 0.8961 & 0.1460 & 0.0125 \TBstrut \\
  & \textsc{Prefix} & \TBstrut \\
  & \textsc{Prefix (Encoder)} & \TBstrut \\
  & \textsc{Composer} & 0.5271 & 0.6434 & 0.7980 & 0.6410 & 0.6277 & 0.7279 & 0.2000 & 0.6133 & 0.7273 & 0.3066 & 0.4125 \TBstrut \\
  
  \hline
  \noalign{\hrule height0.8pt} %%%%=
  
  \textbf{Avg.} & \TBstrut \\
  
  \hline
  \noalign{\hrule height0.8pt} %%%%=
\end{tabular}
\end{adjustbox}
\end{center}
\caption{StylePTB results.}
\label{tab:full}
\end{table*}

==> tables/tab_gpt2.tex <==
\begin{table*}[t!]
\begin{center}
\resizebox{0.9\textwidth}{!}{ % 화이팅입니다...
\begin{tabular}{l ccccccccc c}
  \hline
  \noalign{\hrule height0.8pt} %%%%=
  \multicolumn{1}{l}{\multirow{3}{*}{}} & 
%   \multicolumn{1}{l}{\multirow{3}{*}{}} &
  \multicolumn{8}{c}{Target Composition (number of samples)} &
  \multicolumn{1}{c}{\multirow{3}{*}{Avg.}}
  \TBstrut\\
  \cline{2-9}
  & \shortstack{PPR+PTA \\ (959)} & \shortstack{PPR+ATP \\ (1330)} & \shortstack{TFU+PTA \\ (2967)} & \shortstack{TFU+ATP \\ (2455)} & \shortstack{TPR+PTA \\ (1561)} & \shortstack{TPR+ATP \\ (2163)} & \shortstack{TPA+PTA \\ (1617)} & \shortstack{TPA+ATP \\ (658)} & \DTBstrut \\
%   \hline\noalign{\hrule height0.8pt} 
%   \multirow{1}{*}{\textbf{Support}}
%   & & 959 & 162 & 4492 & 1330 & 178 & 2967 & 2455 & 233 & \TBstrut \\ 
  \hline\noalign{\hrule height0.8pt} 
%   \multirow{2}{*}{\textbf{Full-shot}}
%   & \textsc{Prompt} & 0.9625 & 0.9375 & 0.8912 & 0.8440 & 0.6471 & 0.8880 & 0.8340 & 0.8261 & 0.8759 \TBstrut \\ 
%   & \textsc{Prefix} & 0.8750 & 0.9375 & 0.8796 & 0.7660 & 0.4706 & 0.8533 & 0.7992 & 0.8261 & 0.8399 \TBstrut \\
%   \hline\noalign{\hrule height0.8pt} 
%   \multirow{3}{*}{\textbf{Zero-shot}}   
%   & \textsc{Pipeline} & 0.9750 & 0.9375 & 0.8750 & 0.8156 & 0.8824 & 0.8687 & 0.8263 & 0.8261 & 0.8655\TBstrut \\
%   & \textsc{Prompt} & 0.0375 & 0.7500 & 0.7593 & 0.0142 & 0.2353 & 0.0695 & 0.4054 & 0.8261 & 0.3931 \TBstrut \\
%   & \textsc{Prefix} & & & & & & & & & \TBstrut \\
%   \hline\noalign{\hrule height0.8pt}
%   \multirow{2}{*}
  \textsc{Voice First} & 0.9750	& 0.8156 & 	0.8263 & 0.8687 & 0.8333 & 0.8936 & 0.8571 & 0.6769 & 0.8527268077

 \TBstrut \\
  \textsc{Voice Later} & 0.0250	& 0.0142 & 0.7799 & 0.7954 & 0.7963 & 0.5904 & 0.3000 & 0.4462 &  0.5555202252
  \TBstrut \\

%   \hline\noalign{\hrule height0.8pt} %%%%=
  
%   \textbf{Avg.} & \TBstrut \\
  
  \hline
  \noalign{\hrule height0.8pt} %%%%=
\end{tabular}}
\end{center}
\caption{Comparision between GPT2 and T5}
\label{tab:gpt2}
\end{table*}

==> tables/tab_reproduvibility.tex <==
\begin{table}[t]
\begin{tabular}{lc}
\hline
\multicolumn{1}{c}{\textbf{Criteria}}                                                                                                                                                                                                                                  & \textbf{Self-Check}                                           \\ \hline
\multicolumn{2}{c}{\textbf{For all reported experimental results :}}                                                                                                                                                                                                                                                                   \\ \hline
A clear description of the mathematical setting, algorithm, and/or model                                                                                                                                                                                               & O                                                             \\
\begin{tabular}[c]{@{}l@{}}Submission of a zip file containing source code, with specification of all\\  dependencies, including external libraries, or a link to such resources \\ (while still anonymized) Description of computing infrastructure used\end{tabular} & \begin{tabular}[c]{@{}c@{}}O \\ (Link submitted)\end{tabular} \\
\begin{tabular}[c]{@{}l@{}}The average runtime for each model or algorithm \\ (e.g., training, inference, etc.), or estimated energy cost\end{tabular}                                                                                                                 & O                                                           \\
Number of parameters in each model                                                                                                                                                                                                                                     & O                                                           \\
Corresponding validation performance for each reported test result                                                                                                                                                                                                     & X                                                           \\
Explanation of evaluation metrics used, with links to code                                                                                                                                                                                                             & O                                                             \\ \hline
\multicolumn{2}{c}{\textbf{For all experiments with hyperparameter search :}}                                                                                                                                                                                                                                                          \\ \hline
The exact number of training and evaluation runs                                                                                                                                                                                                                       & 1                                                           \\
Bounds for each hyperparameter                                                                                                                                                                                                                                         & N/A                                                           \\
Hyperparameter configurations for best-performing models                                                                                                                                                                                                               & O                                                           \\
Number of hyperparameter search trials                                                                                                                                                                                                                                 & N/A                                                           \\
\begin{tabular}[c]{@{}l@{}}The method of choosing hyperparameter values (e.g., uniform sampling, \\ manual tuning, etc.) and the criterion used to select among them (e.g., accuracy)\end{tabular}                                                                     & N/A                                                           \\
Summary statistics of the results (e.g., mean, variance, error bars, etc.)                                                                                                                                                                                             & O                                                           \\ \hline
\multicolumn{2}{c}{\textbf{For all datasets used :}}                                                                                                                                                                                                                                                                                   \\ \hline
\begin{tabular}[c]{@{}l@{}}Relevant details such as languages, and number of examples and\\  label distributions\end{tabular}                                                                                                                                          & O                                                           \\
Details of train/validation/test splits                                                                                                                                                                                                                                & O                                                             \\
Explanation of any data that were excluded, and all pre-processing steps                                                                                                                                                                                               & O                                                           \\
A zip file containing data or link to a downloadable version of the data                                                                                                                                                                                               & O                                                           \\
\begin{tabular}[c]{@{}l@{}}For new data collected, a complete description of the data collection \\ process, such as instructions to annotators and methods for quality control.\end{tabular}                                                                          & N/A                                                             \\ \hline
\end{tabular}
\end{table}
\clearpage

==> tables/tab_responsibleNLP.tex <==
\begin{table}[t]
\begin{tabular}{lc}
\hline
\multicolumn{1}{c}{\textbf{responsibleNLPresearch}}                                                                                                                                                                                                                                  & \textbf{Self-Check}                                           \\ \hline
\multicolumn{2}{c}{\textbf{A. For every submission}} \\ \hline
A1. Did you describe the limitations of your work? & O, Sec 8  \\
%\begin{tabular}[c]{@{}l@{}}Submission of a zip file containing source code, with specification of all\\  dependencies, including external libraries, or a link to such resources \\ (while still anonymized) Description of computing infrastructure used\end{tabular} & \begin{tabular}[c]{@{}c@{}}O \\ (Link submitted)\end{tabular} \\

%\begin{tabular}[c]{@{}l@{}}The average runtime for each model or algorithm \\ (e.g., training, inference, etc.), or estimated energy cost\end{tabular} & O \\
A2. Did you discuss any potential risks of your work? & X, Nothing to Expect \\
A3. Do the abstract and introduction summarize the paper’s main claims? & O, Sec 1 \\

\hline
\multicolumn{2}{c}{\textbf{B. Did you use or create scientific artifacts?}}\\ 
\hline

B1. Did you cite the creators of artifacts you used? & O, Sec 4 \\
B2. Did you discuss the license or terms for use and / or distribution of any artifacts? & O \\
B3.\begin{tabular}[c]{@{}l@{}l@{}l@{}} Did you discuss if your use of existing artifact(s) was consistent with their intended use, \\ provided that it was specified? For the artifacts you create, do you specify intended use \\ and whether that is compatible with the original access conditions (in particular, \\ derivatives of data accessed for research purposes should not be used outside \\ of research contexts)?\end{tabular} & O, Sec 4 \\
B4.\begin{tabular}[c]{@{}l@{}} Did you discuss the steps taken to check whether the data that was collected / \\ used  contains any information that names or uniquely identifies individual \\ people  or offensive content, and the steps taken to protect / anonymize it?\end{tabular} &  X, Not Suggested \\
B5.\begin{tabular}[c]{@{}l}Did you provide documentation of the artifacts, e.g., coverage of domains, \\ languages,  and linguistic phenomena, demographic groups represented, etc.?\end{tabular} & O, Sec 4 \\
B6. \begin{tabular}[c]{@{}l}Did you report relevant statistics like the number of examples, details of \\ train / test / dev splits, etc. for the data that you used / created?\end{tabular} & O, Appendix \\
\hline
\multicolumn{2}{c}{C. Did you run computational experiments?} \\ 
\hline
C1. \begin{tabular}[c]{@{}l}Did you report the number of parameters in the models used, the total computational \\ budget (e.g., GPU hours), and computing infrastructure used?\end{tabular} & O, Appendix \\
C2. \begin{tabular}[c]{@{}l}Did you discuss the experimental setup, including hyperparameter \\ search and best-found hyperparameter values?\end{tabular} & O, Appendix \\
C3. \begin{tabular}[c]{@{}l@{}}Did you report descriptive statistics about your results (e.g., error bars around results,\\ summary statistics from sets of experiments), and is it transparent \\whether you are reporting the max, mean, etc. or just a single run?\end{tabular} & O, Appendix \\
C4. \begin{tabular}[c]{@{}l@{}}If you used existing packages (e.g., for preprocessing, for normalization, or for evaluation), \\ did you report the implementation, model, and parameter settings used \\ (e.g., NLTK, Spacy, ROUGE, etc.)?\end{tabular} & O, Sec 4 \\
\hline
\end{tabular}
\end{table}
